Spatiotemporal Event Graphs for Dynamic Scene Understanding

Dynamic scene understanding is the ability of a computer system to interpret and make sense of the visual information present in a video of a real-world scene. In this thesis, we present a series of frameworks for dynamic scene understanding starting from road event detection from an autonomous driving perspective to complex video activity detection, followed by continual learning approaches for the life-long learning of the models. Firstly, we introduce the ROad event Awareness Dataset (ROAD) for Autonomous Driving, to our knowledge the first of its kind. Due to the lack of datasets equipped with formally specified logical requirements, we also introduce the ROad event Awareness Dataset with logical Requirements (ROAD-R), the first publicly available dataset for autonomous driving with requirements expressed as logical constraints, as a tool for driving neurosymbolic research in the area. Next, we extend event detection to holistic scene understanding by proposing two complex activity detection methods. In the first method, we present a deformable, spatiotemporal scene graph approach, consisting of three main building blocks: action tube detection, a 3D deformable RoI pooling layer designed for learning the flexible, deformable geometry of the constituent action tubes, and a scene graph constructed by considering all parts as nodes and connecting them based on different semantics. In a second approach evolving from the first, we propose a hybrid graph neural network that combines attention applied to a graph encoding of the local (short-term) dynamic scene with a temporal graph modelling the overall long-duration activity. Finally, the last part of the thesis is about presenting a new continual semi-supervised learning (CSSL) paradigm.

==> chapters/4_road_r.tex <==
\chapter{ROAD-R: The Autonomous Driving Dataset with Logical Requirements}
\label{chapter:road_r}

\input{chapters/partI/road_r_intro}
\input{chapters/partI/road_r_approach}
\input{chapters/partI/road_r_exp}


\section{Summary of the Chapter}
\label{road_r:sec:future}

We proposed a new learning framework, called learning with requirements, and a new dataset for this task, called ROAD-R. 
We showed that SOTA models most of the times violate the requirements, and how it is possible to exploit the requirements to create models that are compliant with (i.e., strictly satisfy) the requirements while improving their performance.

We envision that requirement specification will become a standard step in the development of machine learning models, to guarantee their safety, as it is in any software development process. In this sense, ROAD-R may be followed by many other datasets with formally specified requirements. 

==> chapters/7_maestro.tex <==
\chapter{Complex Activity Application to Maestro}
\label{chapter:maestro}

\input{chapters/partII/maestro_intro}
\input{chapters/partII/maestro_approach}
\input{chapters/partII/maestro_exp}



==> chapters/partI/road_r_approach.tex <==
\section{Learning with Requirements}\label{road_r:sec:prelim}

In ROAD, the detection of road events requires the following tasks: (i)~identify the bounding boxes,
(ii)~associate with each bounding box a set of labels, and (iii)~form a tube from the identified bounding boxes with the same labels.
Here, we focus on the second task, 
and we formulate it as a multilabel classification problem with requirements.

A {\sl multi-label classification} (MC) problem $\mathcal{P} \,{=}\, (\mathcal{C},\mathcal{X})$ consists of a finite set $\mathcal{C}$ of {\sl labels}, denoted by $A_1, A_2,\ldots$,
and a finite set $\mathcal{X}$ of pairs $(x,y)$, where $x \in \mathbb{R}^D$ $(D \ge 1)$ is a {\sl data point}, and $y \subseteq \mathcal{C}$ is the
{\sl ground truth} of~$x$. The ground truth $y$ associated with a data point $x$ characterizes both the  {\sl positive} and the {\sl negative labels}
 associated with $x$, defined to be $y$ and $\{\neg A: A \in \mathcal{C} \setminus y\}$, respectively. In ROAD-R, a data point corresponds to a bounding box, and each box is labeled with the positive labels representing (i)~the agent performing the actions in the box, (ii) the actions being performed, and (iii) the locations where the actions take place. 
Consider an MC problem $\mathcal{P} = (\mathcal{C},\mathcal{X})$. A {\sl prediction} $p$ is a set of positive and negative labels such that for each label $A \in \mathcal{C}$, either $A \in p$ or $\neg A \in p$.
A {\sl model} $m$ for $\mathcal{P}$ is a function $m(\cdot,\cdot)$ mapping every label $A$ and every datapoint $x$ % \in \mathbb{R}^D$ 
to $[0, 1]$. 
A datapoint $x$ is {\sl predicted} by $m$ to have label $A$ if its {\sl output value} $m(A,x)$ is greater than a user-defined {\sl threshold} $\theta \in [0, 1]$. The  {\sl prediction of $m$ for $x$} is the set $\{A : A \in \mathcal{C}, m(A,x) > \theta\} \cup \{\neg A : A \in \mathcal{C}, m(A,x) \leq \theta\}$ of positive and negative labels.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.90\linewidth, trim={1.5cm 1.1cm 1.0cm 1.3cm},clip]{figures/road_r/main_ex.jpg}
    \caption{
    \!Example of violation of \,$\neg {\text{RedTL}}\,{\vee}\, \neg {\text{GreenTL}}$.}
    \label{fig:redtl}
\end{figure}

An {\sl MC problem with propositional logic requirements} $(\mathcal{P},\Pi)$ consists of an MC problem $\mathcal{P}$ and a finite set $\Pi$ of constraints ruling out non admissible predictions and expressed in propositional logic.

Consider an MC problem with requirements $(\mathcal{P},\Pi)$.
Each requirement delimits the set of  predictions that can be associated with each data point by ruling out those that  violate it. 
A prediction $p$ is 
{\sl admissible} if each constraint $r$ in $\Pi$ is {\sl satisfied} by $p$.
A model $m$ for $\mathcal{P}$ {\sl satisfies} (resp., {\sl violates}) the constraints on a data point $x$ if the prediction of $m$ for $x$ is (resp., is not) admissible. 

The requirement that a traffic light cannot be both red and green  corresponds to the constraint 
 $\{\neg {\text{RedTL}},$ $\neg {\text{GreenTL}}\}$. Any prediction with
$\{\text{RedTL},$ $\text{GreenTL}\}$ 
is non-admissible. An example of such prediction is shown in Fig.~\ref{fig:redtl}.

Given an MC problem with requirements, it is possible to take advantage of the constraints in two different ways: %non mutually exclusive ways: 
\begin{itemize}
    \item they can be exploited during  learning  to teach the model the background knowledge that they express, and 
    \item they can be used as post-processing to turn a non-admissible prediction into an admissible one. 
\end{itemize}
Models in the first and second category are said to have a {\sl constrained loss} (CL) and {\sl constrained output} (CO) respectively.
Constrained loss models have the advantage
that the constraints are deployed during the training phase, and this should result in models (i) with a higher understanding of the problem and a better performance, but still (ii) with no guarantee that no violations will be committed. 
On the other hand, constrained output models
(i) do not exploit the additional knowledge during training, 
but (ii) are guaranteed to have no violations in the final outputs. These two  options are not mutually exclusive (i.e., can be used together), and which one is to be deployed depends also on the extent to which a system is available. For instance, there can be companies that already have  their own models (which can be black boxes) and want to make them compliant with a set of requirements without modifying the model itself. On the other hand, the exploitation of the constraints in the learning phase can be an  attractive option for those who have a good knowledge of the model and want to further improve it.

\begin{table}[t]
    \centering
    \begin{tabular}{lrr}
    \toprule
    \textbf{Statistics} & & \\
    \midrule
      $|\mathcal{C}|$ & 41 \\
       $|\Pi|$ & 243 \\
       $\text{avg}_{r \in \Pi} (|r|)$ & 2.86 \\
       $|\{A \in \mathcal{C} : \exists r \in \Pi. A \in r \}|$ & 41 \\
       $|\{A \in \mathcal{C} : \exists r \in \Pi. \neg{A} \in r \}|$ & 38 \\
       $\text{min}_{A \in \mathcal{C}} (|\{r \in \Pi: \{A,\neg{A}\} \cap r \neq \emptyset\}|)$ & 2 \\        $\text{avg}_{A \in \mathcal{C}} (|\{r \in \Pi: \{A,\neg{A}\} \cap r \neq \emptyset\}|)$ & 16.95 \\ $\text{max}_{A \in \mathcal{C}} (|\{r \in \Pi: \{A,\neg{A}\} \cap r \neq \emptyset\}|)$ & 31 \\
    \bottomrule
    \end{tabular}
    \caption{Constraint statistics. All the constraints have between $2$ and~$15$ positive and negative labels, with an average of $2.86$. All (resp., $38$ of) the labels
    appear positively (resp., negatively) in $\Pi$. Each label 
    appears either positively or negatively between $2$ and $31$ times in $\Pi$, with an average of $16.95$.
    }
    \label{tab:req_stats}
\end{table}

\begin{figure*}[ht!]
\centering
    \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=0.98\textwidth,trim={0 0 7cm 7cm}]{figures/road_r/at_least_one_test.png}
    \caption{Percentage of predictions violating at least one constraint.} % for $\theta \in [0.1,0.9]$.}
    \label{fig:sota-viola}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=0.98\textwidth,trim={0 0 7cm 7cm}]{figures/road_r/avg_viols_per_pred_test.png}
    \caption{Average number of violations committed per prediction.} % for $\theta \in [0.1,0.9]$.}
    \label{fig:sota-violb}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
    \includegraphics[width=0.98\textwidth,trim={0 0 7cm 7cm}]{figures/road_r/perc_violated_constr_test.png}
    \caption{Percentage of constraints violated at least once.} % for $\theta \in [0.1,0.9]$.}
    \label{fig:sota-violc}
    \end{subfigure}
    \caption{ROAD-R and SOTA models. In the $x$-axis, there is the threshold $\theta \in [0.1,0.9]$, step 0.1.}\label{fig:sota}
\end{figure*}


\section{ROAD-R}\label{road_r:sec:roadr}

ROAD-R extends the ROAD dataset\footnote{All the code will be released upon publication. 
ROAD is available at: https://github.com/gurkirt/road-dataset.}
\cite{gurkirt2021} by introducing a set  $\Pi$ of 243 constraints that specify the space of admissible outputs. In order to
improve the usability of our dataset, we write the constraints in a way that allows us to easily express $\Pi$ as a single formula in conjunctive normal form (CNF). The above can be done without any loss in generality, as any propositional formula can be expressed in CNF, and is important because many solvers expects formulas in CNF as input. Thus, each requirement in $\Pi$ has form: 
\begin{equation}\label{eq:req_lit}
l_1 \vee l_2 \vee \cdots \vee l_n\,, 
\end{equation}
where $n \geq 1$, and each $l_i$ is either a negative label $\neg A$ or a positive label~$A$. 
The requirements have been manually specified  following three steps: 
\begin{enumerate}
     \item 
an initial set of constraints $\Pi_1$ was manually created, 
     \item 
a subset $\Pi_2 \subset \Pi_1$ was retained by eliminating all those constraints that were entailed by the others,
     \item 
the final subset $\Pi \subset \Pi_2$ was retained by keeping only those requirements that were always satisfied by the ground-truth labels of the entire ROAD-R dataset.
\end{enumerate}

\begin{table}[t]
    \centering
    \begin{tabular}{rrrr}
    \toprule
%\# labels per rule	&	 \# rules &	avg. neg. labels 	&	avg. pos. labels \\
$n$	&	$|\Pi_n|$ &	$\text{avg}_{r \in \Pi_n} (|r \cap \ov{\mathcal{C}}|)$ 	&	$\text{avg}_{r \in \Pi_n} (|r \cap \mathcal{C}|)$ \\
    \midrule
2	&	215	&	1.995	&	0.005 \\
3	&	5	&	1	&	2 \\
7	&	1	&	1	&	6\\
8	&	6	&	1	&	7\\
9	&	6	&	1	&	8\\
10	&	1	&	0	&	10\\
12	&	1	&	1	&	11\\
14	&	1	&	0	&	14\\
15	&	7	&	1	&	14\\
    \midrule
Total	&	243	&	1.87	&	0.96\\
    \bottomrule
    \end{tabular}
    \caption{Constraint statistics. $\Pi_n$ is the set of constraints $r$ in $\Pi$ with $|r| = n$, i.e., with $n$ positive and negative labels. $\ov{\mathcal{C}} = \{\neg {A} : A \in \mathcal{C}\}$. Each row shows the number of rules $r$ with $|r|=n$, and the average number of negative and positive labels in such rules.}
    \label{tab:req_stats1}
\end{table}

Finally, redundancy in the constraints has been automatically checked with {\sc relsat}\footnote{https://github.com/roberto-bayardo/relsat/}. 
Note that our process of gathering and further selecting the logical requirements follows more closely the software engineering paradigm rather than the machine learning view.
To this end, we ensured that the constraints were consistent with the provided labels from the ROAD dataset in the sense that they were acting as strict conditions to be absolutely satisfied by the ground-truth labels, as emphasized in the third step of the annotation pipeline above.
Tables~\ref{tab:req_stats} and \ref{tab:req_stats1} give a   high-level description of the properties of the set $\Pi$ of constraints. Notice that, with a slight abuse of notation, in the tables we use a set based notation for the requirements. Each requirement of form (\ref{eq:req_lit}) thus becomes 
$$
\{l_1, l_2, \ldots, l_n\}.
$$ Such notation allows us to express the properties of the requirements in a more succinct way.
In addition to the information in the tables, we report that of the 243 constraints, there are two in which all the labels are positive (expressing that there must be at least one agent and that every agent but traffic lights has at least one location), and 214 in which all the labels are negative (expressing mutual exclusion between two labels).  All the constraints with more than two labels have at most one negative label, as they express a one-to-many relation
 between actions and agents (like \rev{in our dataset} ``if something is crossing, then it is a pedestrian or a cyclist'').
Constraints like ``pedestrians should cross at crossings'', which might not be satisfied in practice, are not included.
Additionally embedding such logical constraints would require, e.g., using modal operators and, while it would be an interesting study to see the impact on the model's predictions when adding more complex layers to the expressivity of our logic, we opted for using a simpler logic in this first instance.
This also provides more transparency to the wider research community, as the full propositional logic covers a vast range of applications that do not require extra logical operators. 
% The list with all the 243 requirements, with their natural language explanations, is  in Appendix~\ref{app:req_list},
% Tables~\ref{tab:req_list1}, \ref{tab:req_list2}, and \ref{tab:req_list3}.
Notice that the 243 requirements restrict the number of admissible prediction to $4985868 \sim 5 \times 10^6$,
thus ruling out $(2^{41} - 4985868) \sim 10^{12}$ non-admissible predictions.\footnote{The number of admissible predictions has been computed with relsat: https://github.com/roberto-bayardo/relsat/.}
In principle, the set of admissible predictions can be further reduced by adding other constraints. Indeed, the 243 requirements are not guaranteed to be complete from every possible point of view: as standard in the software development cycle,
the requirement specification process deeply involves the stakeholders of the system (see, e.g., \cite{sommerville}). For example, we decided not to include constraints like ``it is not possible to both move towards and move away", which were not satisfied by all the data points because of errors in the ground truth labels. In these cases, we decided to dismiss the constraint in order to maintain (i) consistency between the knowledge provided by the constraints and by the data points, and (ii) backward compatibility. 

As an additional point, we underline that, even though the annotation of the requirements introduces some overhead in the annotation process, it is also the case that the effort of manually writing 243 constraints (i) is negligible when compared to the effort of manually annotating the 22 videos, and (ii) can improve such last process, e.g., allowing to prevent errors in the annotation of the data points.  




==> chapters/partI/road_r_exp.tex <==
\section{ROAD-R and SOTA Models}
\label{road_r:sec:sota}

As a first step, we ran 6 SOTA temporal feature learning architectures as part of a 3D-RetinaNet model~\cite{gurkirt2021} (with a 2D-ConvNet backbone made of Resnet50~\cite{he2016deep}) for event detection and evaluated 
to which extent constraints are violated. We considered:

\begin{enumerate}
\item {\sl 2D-ConvNet} (C2D)~\cite{wang2018non}:
     a Resnet50-based architecture with an additional temporal dimension for learning features from videos. The extension from 2D to 3D is done by adding a pooling layer over time to combine the spatial features.
\item {\sl Inflated 3D-ConvNet} (I3D)~\cite{carreira2017quo}:
      a sequential learning architecture extendable to any SOTA image classification model (2D-ConvNet based), 
    able to learn continuous spatio-temporal features from the sequence of frames.
\item {\sl Recurrent Convolutional Network} (RCN)~\cite{singh2019recurrent}:
     a 3D-ConvNet model that relies on recurrence for learning the spatio-temporal features at each network level. During the feature extraction phase, RCNs exploit both 2D convolutions across the spatial domain and
    1D convolutions across the temporal domain.  
\item {\sl Random Connectivity Long Short-Term Memory} (RCLSTM) \cite{hua2018traffic}:
     an updated version of LSTM in which the neurons are connected in a stochastic manner, rather than fully connected. In our case, the LSTM cell is used as a bottleneck in Resnet50 for learning the features sequentially.
\item {\sl Random Connectivity Gated Recurrent Unit} (RCGRU)  \cite{hua2018traffic}:
    an alternative version of RCLSTM where the GRU cell is used instead of the LSTM one. GRU makes the process more efficient with fewer parameters than the LSTM.
\item {\sl SlowFast} \cite{feichtenhofer2019slowfast}: a 3D-CNN architecture that contains both slow and fast pathways for extracting the sequential features. A Slow pathway computes the spatial semantics at low frame rate while a Fast pathway processes high frame rate for capturing the motion features. Both of the pathways are fused in a single architecture by lateral connections.
\end{enumerate}
We trained 3D-RetinaNet\footnote{https://github.com/gurkirt/3D-RetinaNets.} using the same hyperparameter settings for all the models: (i) batch size equal to 4, (ii)~sequence length equal to 8, and (iii) image input size equal to $512\times682$. All the models were initialized with the  Kinetics pre-trained weights. An SGD optimizer~\cite{lecun2012} with step learning rate was used. The initial learning rate was set to 0.0041 for all the models except SlowFast, for which it was set to 0.0021 due to the diverse nature of slow and fast pathways. All the models were trained for 30 epochs and the learning rate was made to drop by a factor of 10 after 18 and 25 epochs. The machine used for the experiments has 64 CPUs (2.2 GHz each) and 4 Titan RTX GPUs having 24 GB of RAM each. 

\begin{figure*}[t]

\begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth,height=5.4cm, trim={50pt 30pt 50pt 10pt},clip]{figures/road_r/I3D_2014-06-26-09-31-18_stereo_centre_02_04416.jpg}
         \caption{I3D}
         \label{I3D1}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=5.4cm, trim={20pt 20pt 50pt 10pt},clip]{figures/road_r/C2D_2015-02-06-13-57-16_stereo_centre_01_04630.jpg}
         \caption{C2D}
         \label{C2D1}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=5.4cm, trim={20pt 20pt 50pt 10pt},clip]{figures/road_r/RCGRU_2014-06-26-09-31-18_stereo_centre_02_01536.jpg}
         \caption{RCGRU}
         \label{RCGRU1}
\end{subfigure}

\begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=5.4cm, trim={40pt 20pt 40pt 10pt},clip]{figures/road_r/RCLSTM_2014-06-26-09-31-18_stereo_centre_02_05814.jpg}
         \caption{RCLSTM}
         \label{RCLSTM1}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=5.4cm, trim={20pt 20pt 50pt 10pt},clip]{figures/road_r/RCN_2015-02-06-13-57-16_stereo_centre_01_05131.jpg}
         \caption{RCN}
         \label{RCN1}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth,  height=5.4cm, trim={20pt 20pt 50pt 10pt},clip]{figures/road_r/SlowFast_2014-06-26-09-31-18_stereo_centre_02_05377.jpg}
         \caption{SlowFast}
         \label{Slowfast}
\end{subfigure}
\caption{Examples of violations of $\{\neg{\text{RedTL}},\neg{\text{GreenTL}}\}$.}
\label{fig:violRedTL}
\end{figure*}

To measure the models' performance, we used the {\sl frame mean average precision} (f-mAP), which is the standard metric used for action detection (see, e.g.,~\cite{kalogeiton2017a,li2018map}), with IoU threshold equal to 0.5 and 0.75, indicated as f-mAP@0.5 and f-mAP@0.75,  respectively. 
The results for the SOTA models at IoU threshold 0.5 and 0.75 are reported in Table \ref{tab:map5}, 
column ``SOTA''.

 To measure the extent to which each system violates the constraints, we used the following metrics: 
 \begin{itemize}
     \item the percentage of non-admissible predictions,
     \item the average number of violations committed per prediction, and
     \item  the percentage of constraints violated at least once,
 \end{itemize}
while varying the threshold $\theta$ from 0.1 to 0.9 with step 0.1. 
The results are in Fig.~\ref{fig:sota}, where (to improve readability) we do not plot the values corresponding to $\theta=0.0$ and $\theta=1.0$. For $\theta=0.0$ (resp., $\theta = 1.0$), all the predictions are positive (resp., negative), and thus the corresponding values are (in order) 100\%, 214, and 214/243 (resp., 100\%, 2, and 2/243).


Consider the results in Table \ref{tab:map5}, 
column ``\SOTA'', and in Fig.~\ref{fig:sota}. 
First, note that the performances are not an indicator of the ability of the model to satisfy the constraints. Indeed, higher f-mAPs do not correspond to lower trends in the plots of Fig.~\ref{fig:sota-violb}. For example,
RCGRU performs better than C2D for both IoU = 0.5 and IoU = 0.75, however, its curve is above C2D's in both Figs.~\ref{fig:sota-viola} and~\ref{fig:sota-violb}.
Then, note that the percentage of non-admissible predictions is always very high for every model: at its minimum, for $\theta=0.1$, more than 90\% of the predictions are non-admissible, and this percentage reaches 99\% for $\theta = 0.9$ (see Fig.~\ref{fig:sota-viola}). In addition, most predictions violate roughly two constraints, as shown  by Fig.~\ref{fig:sota-violb}. 
Considering that we are in an autonomous vehicle setting, such results are critical: one of the constraints that is  violated  
by all the baseline models
is $\{\neg{\text{RedTL}}, \neg{\text{GreenTL}}\}$, corresponding to predictions according to which there is a traffic light with both the red and the green lights on. Fig.~\ref{fig:violRedTL} shows an image for each of the SOTA models where such a prediction (for $\theta=0.5$) is made.  
% Appendix~\ref{app:imgs} contains qualitative examples of all the SOTA models making  predictions violating other constraints. 

\begin{table*}[t]
\setlength{\tabcolsep}{2.4pt}
    \centering
    \footnotesize
    \scalebox{0.72}{
    \begin{tabular}{l|c | c c c | c c c | c c c}
    \toprule
     & & \multicolumn{3}{c|}{{\textbf{Constrained Loss (CL)}}} &  \multicolumn{3}{c|}{{\textbf{Constrained Output (CO)}}} &  \multicolumn{3}{c}{{\textbf{Constrained Loss and Output (CLCO)}}} \\
         \textbf{Model}  & \textbf{SOTA} & \textbf{Product} & \textbf{G\"odel} & \textbf{Lukasiewicz}   &  \textbf{\MSbasic} & \textbf{\MSmAP} & \textbf{\MSPred} & \textbf{(P, AP$\times$O)} & \textbf{(G, AP$\times$O)} & \textbf{(L, AP$\times$O)} \\
         \midrule
         C2D & 27.57 & 27.90 \,\,(1)\, & 27.97 \,\,(1)\, & 27.57 (10)  & 27.41 (0.4) & 27.67 (0.9) & 27.69 (0.9) & 27.90 (0.7) & \textbf{28.16} (0.8) & 27.86 (0.9) \\
         I3D & 30.12 & 30.79 (10) & 29.98 (10) &  31.03 (10) & 29.86 (0.4) & 30.15 (0.5) & 30.15 (0.5) & 30.77 (0.9) & 30.02 (0.7) & \textbf{31.21} (0.6) \\
         RCGRU &  30.78 &  30.67 (10) & 29.57 \,\,(1)\, & {31.78} (10) & 30.56 (0.4) & {30.78} (0.5) & {30.78} (0.7) & 30.79 (0.6) & 29.83 (0.9) & \textbf{31.81} (0.5) \\
         RCLSTM & 30.49 & 30.48 (10) & 30.88 \,\,(1)\, & {31.63} (10) & 30.09 (0.4)&  {30.51} (0.7)  &  {30.51} (0.7) & 30.50 (0.5) & 30.90 (0.8) & \textbf{31.65} (0.9)  \\
         RCN & 29.64 & 30.31 (10) & 30.24 (10) & {\textbf{31.02}} (10) & 29.39 (0.4) & 29.80 (0.5)  & {29.82} (0.5) & 30.34 (0.6) & 30.28 (0.8) & \textbf{31.02} (0.5) \\
         SlowFast & 28.79 & 28.54 (10) & {28.91} \,\,(1)\, & 28.47 (10) & 28.51 (0.5) & {28.86} (0.9)  & {28.86} (0.9) & 28.67 (0.9) & \textbf{28.98} (0.5) & 28.56 (0.7) \\
         \midrule
         Avg. Rank & 7.08 & 5.75 &	5.50 &	4.25 & 	9.50 & 	5.75 & 	5.42 & 	4.42 &	4.50 & \textbf{2.83}  \\
    \bottomrule
    \multicolumn{3}{c}{}\\
    \end{tabular}
    }
    \scalebox{0.72}{
    \begin{tabular}{l|c | c c c | c c c | c c c}
    \toprule
     & & \multicolumn{3}{c|}{{\textbf{Constrained Loss (CL)}}} &  \multicolumn{3}{c|}{{\textbf{Constrained Output (CO)}}} &  \multicolumn{3}{c}{{\textbf{Constrained Loss and Output (CLCO)}}} \\
         \textbf{Model}  & \textbf{SOTA} & %Baseline} & 
         \textbf{Product} & \textbf{G\"odel} & \textbf{Lukasiewicz}   &  \textbf{\MSbasic} & \textbf{\MSmAP} & \textbf{\MSPred} & \textbf{(P, AP$\times$O)} & \textbf{(G, AP$\times$O)} & \textbf{(L, AP$\times$O)} \\
         \midrule
  C2D & 12.66 & {13.04} \,\,(1)\, & 12.90 \,\,(1)\, & 12.30 (10) & 12.62 (0.4) & {12.72} (0.9) & {12.72} (0.9) & \textbf{13.05}  (0.8) & 13.01 (0.8) & 12.55 (0.9)  \\
         I3D & 16.29 & {16.47} (10) & 16.19 (10) & 16.32 (10) & 16.22 (0.5) & {16.31} (0.8) & {16.31} (0.8) & \textbf{16.48} (0.6) & 16.20 (0.6) & 16.42 (0.6) \\
         RCGRU &  15.98 & 16.57 (10) & 15.39 \,\,(1)\, & {17.26} (10) & 15.97 (0.4) & 16.02 (0.5) & {16.03} (0.5) & 16.63 (0.6) & 15.63 (0.9) & \textbf{17.27} (0.6) \\
         RCLSTM & {16.64}  & 16.14 (10) & 15.65 \,\,(1)\, & 16.34 (10) & 16.38 (0.4) &  \textbf{16.69} (0.5) & 16.66 (0.7) &  16.15 (0.7)  & 15.67 (0.8) & 16.39 (0.8) \\
         RCN &  15.82 & 16.57 (10) & 16.17 (10) & {17.25} (10) & 15.73 (0.4) & 15.87 (0.8) & {15.89} (0.5) & 16.56 (0.5) & 16.19 (0.9) & \textbf{17.26} (0.9) \\
         SlowFast &  14.40  & 14.84 (10) & 15.38 \,\,(1)\, & 13.80 (10) & 14.33 (0.5) & {14.47} (0.9) & {14.47} (0.9)  & {14.94} (0.9) & \textbf{15.42} (0.5) & 13.84 (0.7) \\
         \midrule
         Avg. Rank & 6.67	& 3.83 &	7.00 & 	5.67 & 	7.83 & 	5.00 &	4.83 & 	\textbf{3.17} & 	6.00 &	4.50  \\
         \bottomrule
\end{tabular}
    }

    \caption{
f-mAP@0.5 (top table) and f-mAP@0.75 (bottom table) 
    for the 
    (i) current SOTA models; (ii) CL models, in parentheses the value of $\alpha$; (iii) CO models, in parenthesis the threshold used to evaluate the admissibility of the predictions; and (iv) CLCO models, in parenthesis the threshold used to evaluate the admissibility of the predictions. \textbf{P},  \textbf{G},  and \textbf{L} stand for the Product, G\"odel, and Lukasiewicz t-norm, respectively.}
    \label{tab:map5}
\end{table*}


\section{ROAD-R and CL, CO, and CLCO Models}\label{road_r:sec:sotacorr}

We now show how it is possible to build CL, CO and CLCO models. In particular, we show how to equip the 6 considered SOTA models with constrained a loss and/or a constrained output. As anticipated in the introduction, we introduce (i) three different methods to build the constrained loss, (ii) three different methods to obtain the constrained output, and (iii) three combinations of constrained loss and constrained output.
Thus, we get 9 models for each SOTA model, for a total of 54. In order to get an overall view of the performance gains produced by each method, we also report the average ranking of the 9 proposed methods and SOTA \cite{demsar2006}, computed as follows: 
\begin{enumerate}
    \item for each row in Table~\ref{tab:map5}, we rank the performances of the 9 CL, CO and CLCO models and of the SOTA model separately: the best performing model gets
the rank 1, the second best gets rank 2, etc., and in case of ties, the rank is split (e.g., the assigned rank is 1.5 if two models have the best performance), and 
\item for each column, %(i.e., model), 
we
take the average of the rankings computed in the previous step.
\end{enumerate}
See Table \ref{tab:map5} 
for f-mAP@0.5, f-mAP@0.75 and average rankings.
In the table, for each row the best results  are in bold. 
The details of the implemented models with constrained loss, constrained output, and  both constrained loss and constrained output is given in the three paragraphs below. 


\paragraph{Constrained Loss.} To constrain the loss, we take inspiration from the approaches proposed in~\cite{diligenti2017icmla,diligenti2017semantic}, and we %incorporate the constraints in the loss. We 
train the models using the standard localization and classification losses, to which we add a regularization term. This last term represents the degree of satisfaction of the constraints in $\Pi$ and has the form: 
$$
\mathcal{L}_{\Pi} = \alpha \sum\nolimits_{i=1}^{|\Pi|} (1 - t(r_i)), 
$$
where $r_i$ represents the $i$th constraint in $\Pi$, $t(r_i)$ represents the fuzzy logic relaxation of $r_i$, and $\alpha$ is a hyperparameter ruling the weight of the regularization term (the higher $\alpha$ is, the more relevant the term corresponding to the constraints becomes, up to the limit case in which $\alpha \to \infty$ and the constraints become hard \cite{diligenti2017semantic}). 
We considered $\alpha \in \{1, 10, 100\}$ and the three fundamental t-norms:
\begin{enumerate}
    \item Product t-norm, 
    \item G\"odel t-norm, and
    \item Lukasiewicz t-norm
\end{enumerate}
as fuzzy logic relaxations (see e.g., \cite{metcalfe2005}).

The best results for f-mAP@0.5 and f-mAP@0.75 while varying $\alpha$ are in Table~\ref{tab:map5},  columns Product, G\"odel, and Lukasiewicz. As can be seen, SOTA  never achieves the best average ranking, even when compared with only the three CL methods. Of these, Lukasiewicz (for IoU = 0.5) and Product (for IoU = 0.75) have the best ranking, though for some model and IoU, the best performances are obtained with G\"odel. In only one case (for RCLSTM at IoU = 0.75), the 
SOTA model performs better than the CL models. Also notice that the best performances are never obtained with $\alpha=100$, and that we never get any significant reduction in the number of predictions violating the constraints.


\paragraph{Constrained Output.} \label{sec:sotacorr}

We now consider the problem of how to correct a prediction $p$ whose admissibility is evaluated at a given threshold $\theta$. The first observation is that determining the existence of an admissible prediction is an intractable problem: indeed, this is just a reformulation of the satisfiability problem in propositional logic, which is well known to be NP-complete. Despite this, we want to correct any non-admissable prediction $p$ in such a way that (i) the final prediction is admissible, and (ii) the performance of the final model either improves or remains unaltered. 

In order to achieve the above, 
we first test the policy of trying to correct as few labels as possible. 
%correcting any  it does not perform unnecessary corrections.
More precisely, for each prediction $q$, $(p \setminus q)$ is the set of positive and negative predictions on which $q$ differs from $p$. Then, we can compute the admissible prediction $q$ with the minimum number of differences, i.e., such that $| p \setminus q |$ is minimal. We call such policy {\sl Minimal Distance} (MD). Unfortunately, no polynomial time algorithm is known to solve this problem.

%  \begin{theorem}\label{th:one}
%  Let $(\mathcal{P},\Pi)$ be an MC problem with requirements. Let $p$ be a prediction. For each positive $d$, determining the existence of an admissible prediction $q$ such that $\mid p \setminus q \mid \le d$ is an NP-complete problem.
%   \end{theorem}
% The theorem is an easy consequence of Proposition 1 in \cite{DBLP:BailleuxM06}. 
% %From a practical perspective, 
% In order to be able to solve the problem in practice, we formulate the problem of finding an admissible prediction with minimal $\mid p \setminus q \mid$ as a weighted partial maximum satisfiability (PMaxSAT) problem of a set of clauses\footnote{In our setting, a {\sl clause} is a disjunction of literals, and a {\sl literal} is either a positive label or its negation, representing the corresponding negative label. A clause is {\sl unit} if it consists of a single literal.} (see, e.g., \cite{DBLP:LiM09}) in which
% \begin{enumerate}
% \item each constraint in $\Pi$ corresponds to a clause marked as hard, and
% \item each positive and negative prediction in $p$ corresponds to a unit clause marked as soft with unitary weight.
% \end{enumerate}
% This allows us to use the very efficient solvers publicly available for PMaxSat problems. In particular, in our experiments we used  MaxHS~\cite{hickey2019}, and running times were in the order of  $10^{-3}$s at most.
% As intended, since we assign all labels unitary weight, MaxHS  
% returns the admissible prediction $q$ with as few as possible labels flipped.
% Notice that flipping the $i$th label amounts to changing its output value $o_i$ from a value below the threshold to another value $f(o_i)$ above the threshold or vice versa. In all our experiments, we considered (i)
% $f(o_i) = \theta + \epsilon$, if $o_i < \theta$, and (ii) $f(o_i) = \theta - \epsilon$, otherwise ($\epsilon= 10^{-3}$). In this way, assuming $o_i \leq \theta$ (i.e., the label is negatively predicted and then flipped positive), we expect $f(o_i)$ to be lower (but still higher than $\theta$) than the output values of the non-flipped, positively predicted labels. It is done analogously for the case $o_i > \theta$.
% We tested this approach with all the thresholds $\theta$ from 0.1 to 0.9 with step 0.1, 
% and the resulting f-mAP@0.5 and f-mAP@0.75 for the best threshold are reported in Table~\ref{tab:map5},
% column MD. As we can see from  the table, despite the fact that we are minimizing the number of corrections, the results obtained by the CO-MD model are always worse than the ones obtained by the SOTA models. We can hence conclude that adding such post-processing has a detrimental effect on the models' performance.

% Thus, we need alternative policies to correct a non-admissable prediction $p$. We generalise the problem by assigning a positive weight $w_i$ (representing the cost of correcting the $i$th  label in $p$) and then computing the admissible prediction $q$ that minimizes $\sum_{i=1}^{41} w_i$. More precisely, for every prediction $q$, $cost(p,q) = \sum_{i \in \mathcal{I}} w_i$, $\mathcal{I}$ being the set of indexes of the labels in $(p \setminus q)$. Then, we can compute the admissable prediction $q$ such that $cost(p,q)$ is minimal.   Being it a generalization of the problem above, no polynomial time algorithm is known to solve this problem.


%  \begin{theorem}
%  Let $(\mathcal{P},\Pi)$ be an MC problem with requirements. Let $p$ be a prediction and let $w_i$ be the cost of correcting the $i$th label in $p$.
%  For each positive $d$, determining the existence of an admissible prediction $q$ such that $cost(p,q) \le d$ is an NP-complete problem.
%   \end{theorem}
% This is an easy consequence of Theorem~\ref{th:one}. Luckily, we can again formulate the problem as a PMaxSAT problem in which: 
% \begin{enumerate}
%     \item each constraint in $\Pi$ corresponds to a clause marked as hard, and
%     \item for each $i$ ($1 \le i \le 41$), the prediction in $p$ for the $i$th label corresponds to a unit clause having weight $w_i$. 
% \end{enumerate}
% Given the above two formulation, we tested two policies: 
% \begin{enumerate}
%      \item {\sl Average Precision based} (\MSmAP), in which each $w_i$ is equal to the average precision $AP_i$ of the $i$th label, and
%     \item {\sl Average Precision and Output based} (\MSPred), in which each $w_i = AP_i \times c_i$, where $c_i$ is equal to (i) the output $o_i$ of the model for the $i$th label if $o_i > \theta$, and (ii) $(1-o_i)$, otherwise.
% \end{enumerate}
% Differently from the MD policy, in order to take a decision, these policies take into
% account the reliability of the output $o_i$ of the model for the $i$th label. 
% We again tested the two policies with all the thresholds $\theta$ from 0.1 to 0.9 with step 0.1, 
% and the resulting f-mAP@0.5 and f-mAP@0.75 for the best threshold are reported in Table~\ref{tab:map5}, 
% columns \MSmAP{}, and \MSPred.
% Comparing the predictions of the SOTA models with the CO-\MSmAP{} and the CO-\MSPred{} models, we can see that flipping the variables taking into account the average precision (i) never leads to worse performances than the ones of the  SOTA models, and (ii) for IoU = 0.75, correcting the output of RCLSTM with \MSmAP{} and \MSPred{}  gives the best and second best performance in the row. 
% Notice that the differences in the performances between \MSmAP{} and \MSPred{} are always negligible, \MSPred{} being better than \MSmAP{} more often.
% The average rankings are in line with the above statements.



==> chapters/partI/road_r_intro.tex <==
\section{Introduction} \label{road_r:intro}

In this chapter, we introduce logical constraints to our ROad event Awareness Dataset (ROAD) (explained in Chapter \ref{chapter:road}). The main intuition behind these logical constraints is that neural networks have proven to be very powerful at computer vision tasks. However, they often exhibit unexpected behaviours, violating known requirements and expressing background knowledge.  This calls for models (i) able to learn from the requirements, and (ii) be guaranteed to be compliant with the requirements  themselves. Unfortunately, the development of such models is hampered by the lack of datasets equipped with formally specified requirements. Therefore, we introduce the ROad event Awareness Dataset with logical Requirements (ROAD-R), the first publicly available dataset for autonomous driving with requirements expressed as logical constraints. 
Given ROAD-R, we show that current state-of-the-art models often violate its logical constraints and that it is possible to exploit them to create models that (i) have a better performance, and (ii) are guaranteed to be compliant with the requirements themselves.

\subsection{Motivation}
Neural networks have proven to be incredibly powerful at processing low-level inputs, and for this reason, they have been extensively applied to computer vision tasks, such as image classification, object detection, and action detection. However, they can exhibit unexpected behaviors, contradicting known requirements and expressing background knowledge. This can have dramatic consequences, especially in safety-critical scenarios such as autonomous driving. To address the problem, models should  (i) be able to learn from the requirements, and (ii) be guaranteed to be compliant with the requirements  themselves. Unfortunately, the development of such models is hampered by the lack of datasets equipped with formally specified requirements.
A notable exception is given by  hierarchical multi-label classification (HMC) problems (see, e.g., \cite{vens2008,schietgat2010,cerri2018}) in which datasets are  provided with  simple binary constraints of the form $(A \to B)$ stating that label $B$ must be predicted whenever label $A$ is predicted.

\subsection{Objective}
In this chapter, we generalize HMC problems by introducing {\sl multi-label classification problems with (full) propositional logic requirements}. Thus,   given a multi-label classification problem with labels $A$, $B$, and $C$, we can, for example, write the requirement: 
$$
(\neg A \wedge B) \vee C,
$$
stating that for each data point in the dataset either the label $C$ is predicted, or $B$ but not $A$ are predicted. 

Then, we present the ROad event Awareness Dataset with logical Requirements (ROAD-R), the first 
publicly available dataset for autonomous driving with requirements expressed as logical constraints.  ROAD-R extends the ROAD dataset \cite{gurkirt2021}, which consists of 22 relatively long ($\sim\!\!\!~8$ minutes each) videos annotated with {\sl road events}. A road event corresponds to a tube, i.e., a sequence of frame-wise bounding boxes linked in time. Each bounding box is labeled with a subset of the 41 labels specified in Table \ref{tab:labels}. The goal is to predict the set of labels associated with each bounding box.  
We manually annotated ROAD-R with 243 constraints, each  verified to hold for each bounding box. A typical constraint is thus ``a traffic light cannot be red and green at the same time'', while there are no constraints like ``pedestrians should cross at
crossings”, which should always be satisfied in theory, but which might not be in real-world scenarios.

\begin{table}[t]

    \centering
    \begin{tabular}{l l l}
    \toprule
         \textbf{Agents} & \textbf{Actions} & \textbf{Locations} \\
    \midrule
    Pedestrian & Move away & AV lane \\
    Car & Move towards & Outgoing lane\\
    Cyclist & Move & Outgoing cycle lane \\
    Motorbike & Brake &  Incoming lane\\
    Medium vehicle & Stop & Incoming cycle lane \\ 
    Large vehicle & Indicating left & Pavement\\
    Bus & Indicating right & Left pavement \\
    Emergency vehicle & Hazards lights on & Right pavement\\
    AV traffic light & Turn left & Junction\\
    Other traffic light & Turn right & Crossing location \\
                        & Overtake & Bus stop \\
                        & Wait to cross & Parking\\
                        & Cross from left \\
                        & Cross from right \\
                        & Crossing \\
                        & Push object \\
                        & Red traffic light \\
                        & Amber traffic light \\
                        & Green traffic light \\
    \bottomrule
    \end{tabular}
    \caption{ROAD labels.}
    \label{tab:labels}
\end{table}

Given ROAD-R, we considered 6 current state-of-the-art (SOTA) models, and we showed that they are not able to learn the requirements  just from the data points, as more than 90\% of the times, they produce predictions that violate the constraints. Then, we
faced the problem of how to leverage the additional knowledge provided by constraints with the goal of (i)~improving their performance, measured by the frame mean average precision (f-mAP) at intersection over union (IoU) thresholds 0.5 and 0.75; see, e.g.,~\cite{kalogeiton2017a,li2018map}, and (ii) guaranteeing that they are compliant with the constraints. 
To achieve the above two goals, three new models are proposed including CL models (with a {\sl constrained loss}),  CO models (with a {\sl constrained output}), and CLCO models (with both a constrained loss and a constrained output).

In particular, we consider three different ways to build CL (resp.,  CO, CLCO) models. More specifically, we run the $9 \times 6$ models obtained by equipping the 6 current SOTA models with a constrained loss and/or a constrained output, and we show that it is always possible to
\begin{enumerate}
    \item improve the performance of each SOTA model, and 
    \item be compliant with (i.e., strictly satisfy) the constraints. 
\end{enumerate}
Overall, the best performing model (for IoU = 0.5 and also IoU = 0.75) is CLCO-RCGRU, i.e., the SOTA model RCGRU equipped with both constrained loss and constrained output: CLCO-RCGRU (i)~always satisfies the requirements  and (ii)~has f-mAP = 31.81 for IoU = 0.5, and f-mAP = 17.27 for IoU = 0.75.
On the other hand, the standard RCGRU model 
(i)~produces predictions that violate the constraints at least 92\% of the times,
and (ii) has f-mAP = 30.78 for IoU = 0.5 and f-mAP = 15.98 for IoU = 0.75. 


\subsection{Main Contributions}
The main contributions of this chapter are thus as follows: 
\begin{enumerate}
\item A multi-label classification problems with propositional logic requirements.
\item Introduction of ROAD-R, which is the first publicly available dataset whose requirements are expressed in full propositional logic.
\item Considered 6 SOTA models and show that on ROAD-R,  they produce predictions violating the requirements more than $\sim$90\% of the times, 
\item Propose new models with a constrained loss and/or constrained output, and conduct an extensive experimental analysis and show that, with our new models, it is always possible to improve the performance of the SOTA models and satisfy the requirements.
\end{enumerate}

\paragraph{Related publications:}
The work of this chapter appeared in IJCAI 2022 Workshop on Artificial Intelligence for Autonomous Driving (AI4AD 2022)\footnote{\url{https://learn-to-race.org/workshop-ai4ad-ijcai2022/}} and IJCLR 2022 the International Joint Conference on Learning and Reasoning \cite{giunchiglia2022road}. This work received \textbf{the best paper award}  at IJCAI 2022 AI4AD and won \textbf{the best student paper award} at IJCLR 2022. The dissertation's author was the co-author in both papers. The main contribution of the dissertation's author to this project is providing the vision baselines for on ROAD dataset for logical constraint. All the resources of this project are publically available and are accessed from \emph{code}\footnote{\url{https://github.com/EGiunchiglia/ROAD-R}}, video\footnote{\url{https://www.youtube.com/watch?v=_-Ll5d1VQXY}}.

\paragraph{Outline:} 

The rest of this chapter is organized as follows. After the introduction to the problem, we present ROAD-R (Section \ref{road_r:sec:roadr}), followed by the evaluation of the SOTA models (Section \ref{road_r:sec:sota})  and of the SOTA models incorporating the requirements (Section \ref{road_r:sec:sotacorr}) on ROAD-R. We end the chapter with the summary and outlook (Section \ref{road_r:sec:future}).

==> chapters/partII/maestro_approach.tex <==
\section{Overview of the approach} 
\label{maestro:approach}


==> chapters/partII/maestro_exp.tex <==
\section{Experiments} 
\label{maestro:exp}


==> chapters/partII/maestro_intro.tex <==
\section{Introduction} 
\label{maestro:intro}


==> pads/epiface.tex <==
\newpage
\begin{center}	
{\large
\textbf{Epiface}
}
\end{center}
\addcontentsline{toc}{chapter}{Epiface}    
\vspace{1cm}
``It does not always end the way we wish it had.''

I would like to start the end by saying thank you to the readers. You got so far and I hope along the way you enjoyed and learned few new things.

Now, in this thesis we have extensivly discussed and proposed solutions for spatiotemopral action detection problem. Towards the end we also learned about prediction and causal representations.

==> pads/titlepage.tex <==
\begin{titlepage}

	\begin{minipage}{0.9\textwidth}
	%\vspace{2cm}
	\end{minipage}
	
	\begin{center}
		\Large
		\textbf{ONLINE SPATIOTEMPORAL ACTION DETECTION AND PREDICTION VIA CAUSAL REPRESENTATIONS} 
		%Towards Casual Action Tube Prediction}
	\end{center}	
		
	\vspace{2.5cm}
		
		
	\begin{center}		
		\Large
		{GURKIRT SINGH}
	\end{center}
	
	\vspace{0.5in}
	
	\begin{center}
	Ph.D.
\end{center}
% 		%\Large
%             A Thesis Submitted in Partial Fulfilment\\
%             of the Requirements for the Degree of \\
%             Doctor of Philosophy    \\
%             in \\
% 	Computer Science and Mathematics
% 	\end{center}
	
	
	
% 	\vspace{0.3in}

% 	\begin{center}
% 	%Department of Computing and Communication Technologies\\
% 	Visual Artificial Intelligence Lab\\
% 	School of Engineering, Computing and Mathematics\\
% 	Oxford Brookes University
% 	\end{center}
	
	\vspace{0.5in}

	
% 	\begin{center}
% 	Supervised by :\\
% 	Prof. Fabio Cuzzolin and Prof. Nigel Crook \\
% % 		 \footnotesize           
% % 		A dissertation submitted to the Faculty of Technology in partial fulfilment \\
% % 		of the requirements of the award of Doctor of Philosophy.  
% 	\end{center}

% 	\vspace{0.1in}
	
	\begin{center}		
		\small
		2019
	\end{center}
	
\end{titlepage}

